The Atacama Cosmology Telescope: Calibration with WMAP Using Cross-Correlations

We present a new calibration method based on cross-correlations with WMAP and apply it to data from the Atacama Cosmology Telescope (ACT). ACT's observing strategy and map making procedure allows an unbiased reconstruction of the modes in the maps over a wide range of multipoles. By directly matching the ACT maps to WMAP observations in the multipole range of 400 < ell < 1000, we determine the absolute calibration with an uncertainty of 2% in temperature. The precise measurement of the calibration error directly impacts the uncertainties in the cosmological parameters estimated from the ACT power spectra. We also present a combined map based on ACT and WMAP data that has high signal-to-noise over a wide range of multipoles.

==> authors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WARNING: This LaTeX block was generated automatically by ../etc/authors.py
% Do not change by hand: your changes will be lost.

\author{
Amir~Hajian\altaffilmark{1,2,3},
Viviana~Acquaviva\altaffilmark{4,2},
Peter~A.~R.~Ade\altaffilmark{5},
Paula~Aguirre\altaffilmark{6},
Mandana~Amiri\altaffilmark{7},
John~William~Appel\altaffilmark{3},
L.~Felipe~Barrientos\altaffilmark{6},
Elia~S.~Battistelli\altaffilmark{11,7},
J.~Richard~Bond\altaffilmark{1},
Ben~Brown\altaffilmark{12},
Bryce~Burger\altaffilmark{7},
Jay~Chervenak\altaffilmark{13},
Sudeep~Das\altaffilmark{14,3,2},
Mark~J.~Devlin\altaffilmark{9},
Simon~R.~Dicker\altaffilmark{9},
W.~Bertrand~Doriese\altaffilmark{15},
Joanna~Dunkley\altaffilmark{16,3,2},
Rolando~D\"{u}nner\altaffilmark{3},
Thomas~Essinger-Hileman\altaffilmark{3},
Ryan~P.~Fisher\altaffilmark{3},
Joseph~W.~Fowler\altaffilmark{3},
Mark~Halpern\altaffilmark{7},
Matthew~Hasselfield\altaffilmark{7},
Carlos~Hern\'andez-Monteagudo\altaffilmark{17},
Gene~C.~Hilton\altaffilmark{15},
Matt~Hilton\altaffilmark{18,19},
Adam~D.~Hincks\altaffilmark{3},
Ren\'ee~Hlozek\altaffilmark{16},
Kevin~M.~Huffenberger\altaffilmark{20},
David~H.~Hughes\altaffilmark{21},
John~P.~Hughes\altaffilmark{4},
Leopoldo~Infante\altaffilmark{6},
Kent~D.~Irwin\altaffilmark{15},
Jean~Baptiste~Juin\altaffilmark{6},
Madhuri~Kaul\altaffilmark{9},
Jeff~Klein\altaffilmark{9},
Arthur~Kosowsky\altaffilmark{12},
Judy~M~Lau\altaffilmark{22,23,3},
Michele~Limon\altaffilmark{24,9,3},
Yen-Ting~Lin\altaffilmark{25,2,6},
Robert~H.~Lupton\altaffilmark{2},
Tobias~A.~Marriage\altaffilmark{2,8},
Danica~Marsden\altaffilmark{9},
%Krista~Martocci\altaffilmark{26,3},
Phil~Mauskopf\altaffilmark{5},
Felipe~Menanteau\altaffilmark{4},
Kavilan~Moodley\altaffilmark{18,19},
Harvey~Moseley\altaffilmark{13},
Calvin~B~Netterfield\altaffilmark{27},
Michael~D.~Niemack\altaffilmark{15,3},
Michael~R.~Nolta\altaffilmark{1},
Lyman~A.~Page\altaffilmark{3},
Lucas~Parker\altaffilmark{3},
Bruce~Partridge\altaffilmark{10},
%Hernan~Quintana\altaffilmark{6},
Beth~Reid\altaffilmark{28,3},
Neelima~Sehgal\altaffilmark{22},
Blake~D.~Sherwin\altaffilmark{3},
Jon~Sievers\altaffilmark{1},
David~N.~Spergel\altaffilmark{2},
Suzanne~T.~Staggs\altaffilmark{3},
Daniel~S.~Swetz\altaffilmark{9,15},
Eric~R.~Switzer\altaffilmark{26,3},
Robert~Thornton\altaffilmark{9,29},
Hy~Trac\altaffilmark{30,31},
Carole~Tucker\altaffilmark{5},
Ryan~Warne\altaffilmark{18},
%Grant~Wilson\altaffilmark{31},
Ed~Wollack\altaffilmark{13},
Yue~Zhao\altaffilmark{3}
}
\altaffiltext{1}{Canadian Institute for Theoretical Astrophysics, University of Toronto, Toronto, ON, Canada M5S 3H8}
\altaffiltext{2}{Department of Astrophysical Sciences, Peyton Hall, 
Princeton University, Princeton, NJ USA 08544}
\altaffiltext{3}{Joseph Henry Laboratories of Physics, Jadwin Hall,
Princeton University, Princeton, NJ, USA 08544}
\altaffiltext{4}{Department of Physics and Astronomy, Rutgers, 
The State University of New Jersey, Piscataway, NJ USA 08854-8019}
\altaffiltext{5}{School of Physics and Astronomy, Cardiff University, The Parade, Cardiff, Wales, UK CF24 3AA}
\altaffiltext{6}{Departamento de Astronom{\'{i}}a y Astrof{\'{i}}sica, 
Facultad de F{\'{i}}sica, Pontific\'{i}a Universidad Cat\'{o}lica de Chile,
Casilla 306, Santiago 22, Chile}
\altaffiltext{7}{Department of Physics and Astronomy, University of
British Columbia, Vancouver, BC, Canada V6T 1Z4}
\altaffiltext{8}{Dept. of Physics and Astronomy, The Johns Hopkins University, 3400 N. Charles St., Baltimore, MD 21218-2686}
\altaffiltext{9}{Department of Physics and Astronomy, University of
Pennsylvania, 209 South 33rd Street, Philadelphia, PA, USA 19104}
\altaffiltext{10}{Department of Physics and Astronomy, Haverford College,
Haverford, PA, USA 19041}
\altaffiltext{11}{Department of Physics, University of Rome ``La Sapienza'', 
Piazzale Aldo Moro 5, I-00185 Rome, Italy}
\altaffiltext{12}{Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh, PA, USA 15260}
\altaffiltext{13}{Code 553/665, NASA/Goddard Space Flight Center,
Greenbelt, MD, USA 20771}
\altaffiltext{14}{Berkeley Center for Cosmological Physics, LBL and
Department of Physics, University of California, Berkeley, CA, USA 94720}
\altaffiltext{15}{NIST Quantum Devices Group, 325
Broadway Mailcode 817.03, Boulder, CO, USA 80305}
\altaffiltext{16}{Department of Astrophysics, Oxford University, Oxford, 
UK OX1 3RH}
\altaffiltext{17}{Max Planck Institut f\"ur Astrophysik, Postfach 1317, 
D-85741 Garching bei M\"unchen, Germany}
\altaffiltext{18}{Astrophysics and Cosmology Research Unit, School of
Mathematical Sciences, University of KwaZulu-Natal, Durban, 4041,
South Africa}
\altaffiltext{19}{Centre for High Performance Computing, CSIR Campus, 15 Lower
Hope St. Rosebank, Cape Town, South Africa}
\altaffiltext{20}{Department of Physics, University of Miami, Coral Gables, 
FL, USA 33124}
\altaffiltext{21}{Instituto Nacional de Astrof\'isica, \'Optica y 
Electr\'onica (INAOE), Tonantzintla, Puebla, Mexico}
\altaffiltext{22}{Kavli Institute for Particle Astrophysics and Cosmology, Stanford
University, Stanford, CA, USA 94305-4085}
\altaffiltext{23}{Department of Physics, Stanford University, Stanford, CA, 
USA 94305-4085}
\altaffiltext{24}{Columbia Astrophysics Laboratory, 550 W. 120th St. Mail Code 5247,
New York, NY USA 10027}
\altaffiltext{25}{Institute for the Physics and Mathematics of the Universe, 
The University of Tokyo, Kashiwa, Chiba 277-8568, Japan}
\altaffiltext{26}{Kavli Institute for Cosmological Physics, 
Laboratory for Astrophysics and Space Research, 5620 South Ellis Ave.,
Chicago, IL, USA 60637}
\altaffiltext{27}{Department of Physics, University of Toronto, 
60 St. George Street, Toronto, ON, Canada M5S 1A7}
\altaffiltext{28}{ICREA \& Institut de Ciencies del Cosmos (ICC), University of
Barcelona, Barcelona 08028, Spain}
\altaffiltext{29}{Department of Physics , West Chester University 
of Pennsylvania, West Chester, PA, USA 19383}
\altaffiltext{30}{Harvard-Smithsonian Center for Astrophysics, 
Harvard University, Cambridge, MA, USA 02138}
\altaffiltext{31}{Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213}
%\altaffiltext{31}{Department of Astronomy, University of Massachusetts, 
%Amherst, MA, USA 01003}
%\altaffiltext{31}{Southern African Astronomical Observatory, Observatory Road,
%Observatory 7925, South Africa}

% End auto-generated block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

